On Minimizing the Number of Running Buffers for Tabletop Rearrangement

For tabletop rearrangement problems with overhand grasps, storage space outside the tabletop workspace, or buffers, can temporarily hold objects which greatly facilitates the resolution of a given rearrangement task. This brings forth the natural question of how many running buffers are required so that certain classes of tabletop rearrangement problems are feasible. In this work, we examine the problem for both the labeled (where each object has a specific goal pose) and the unlabeled (where goal poses of objects are interchangeable) settings. On the structural side, we observe that finding the minimum number of running buffers (MRB) can be carried out on a dependency graph abstracted from a problem instance, and show that computing MRB on dependency graphs is NP-hard. We then prove that under both labeled and unlabeled settings, even for uniform cylindrical objects, the number of required running buffers may grow unbounded as the number of objects to be rearranged increases; we further show that the bound for the unlabeled case is tight. On the algorithmic side, we develop highly effective algorithms for finding MRB for both labeled and unlabeled tabletop rearrangement problems, scalable to over a hundred objects under very high object density. Employing these algorithms, empirical evaluations show that random labeled and unlabeled instances, which more closely mimics real-world setups, have much smaller MRBs.

==> 09-discussion.tex <==
\textcolor{red}{There are some interesting, remaining open problems related to \mrb. On the structural side, while \lrbm in general is proven to be NP-Hard, the computational intractability of either \lrbm with uniform cylinders or \urbm in general is still unknown.
As for bounds, the upper bound of \mrb for \lrbm with uniform cylinders is missing.} 

\textcolor{red}{In terms of random instances, as the environment density $\rho$ grows, 
previous works have seen a phase transition in \vsp on random geometric graphs\cite{diaz2000convergence}\cite{penrose2000vertex}. 
These results motivate us to seek for the phase transition in \mrb with random uniform disk arrangements as well.}

==> 20-app.tex <==
\subsection{Proofs and Proof Sketches}
\begin{proof}[Proof sketch of Proposition~\ref{p:udg}]
The bipartite and planar part come directly from the problem setup. Since we 
work with uniform cylinders which have uniform disc base, one disc may only 
touch six non-overlapping discs and non-trivially intersect at most five 
non-overlapping discs. 
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lemma:adjacent}]
If there is a $j, 1\leq j \leq m$, such that only one of the goal vertices in vertex pairs 
$p_{i,j}$ and $p_{i+1, j}$ is filled (Fig. \ref{fig:LemmaProof}(a)), then the start 
vertex in the other vertex pair must be cleared. Therefore, $c_i+c_{i+1}\geq 1$.

On the other hand, if, for each $j, 1\leq j \leq m$, both or neither of the goal vertices 
in $p_{i,j}$ and $p_{i+1,j}$ is filled, then there is a $j, 1 \leq j \leq m-1$, such that both 
goal vertices in $p_{i,j}$ and $p_{i+1,j}$ are filled but neither of those in $p_{i,j+1}$ and $p_{i+1,j+1}$ is filled (Fig.~\ref{fig:LemmaProof}(b)) or the opposite 
(Fig.~\ref{fig:LemmaProof}(c)). Then, for the vertex pairs whose goal vertices are not filled, 
say $p_{i,j+1}$ and $p_{i+1, j+1}$, one of their start vertices is a neighbor of the filled 
goal in $p_{i,j}$ and $p_{i,j+1}$. Therefore, at least one of the start vertices in $p_{i, j+1}$ 
and $p_{i+1,j+1}$ is a cleared vertex. And thus, $c_i+c_{i+1}\geq 1$.

\begin{figure}[h!]
    \centering
    \vspace{5mm}
    \begin{overpic}
    [width = 0.30\textwidth]{lemma_cases-eps-converted-to.pdf}
    \put(0, 38){{\small $p_{i,j}$}}
    \put(11, 38){{\small $p_{i+1,j}$}}
    
    \put(37, 51){{\small $p_{i,j}$}}
    \put(49, 51){{\small $p_{i+1,j}$}}
    \put(34, -3){{\small $p_{i,j+1}$}}
    
    \put(89, 51){{\small $p_{i+1,j}$}}
    \put(70, -3){{\small $p_{i,j+1}$}}
    \put(89, -3){{\small $p_{i+1,j+1}$}}
    
    \put(8, -9.5){{\small $(a)$}}
    \put(44, -9.5){{\small $(b)$}}
    \put(85, -9.5){{\small $(c)$}}
    \end{overpic}
    \vspace{6mm}
    \caption{Some cases discussed in the lemma~\ref{lemma:adjacent}. The green and cyan nodes represent the start and goal vertices in the dependency graph. Specifically, the cyan nodes with a dot inside represent the filled vertices and the green nodes with a cross inside represent the cleared vertices. (a) When only one goal vertex in $p_{i,j}$ and $p_{i+1, j}$ is filled up, the start vertex in the other vertex pair is a cleared vertex. (b) When both goal vertices in $p_{i,j}$ and $p_{i+1,j}$ are filled but neither of those in $p_{i,j+1}$ and $p_{i+1,j+1}$ is filled, one of the start vertices $p_{i,j+1}$ and $p_{i+1,j+1}$ is a cleared vertex. (c) The opposite case of (b).}
    \label{fig:LemmaProof}
\end{figure}
\end{proof}

\begin{proof}[Proof of Lemma~\ref{l:urbm-lower}]
We show that there are $\Omega(m)$ cleared vertices when $\lfloor n/3 \rfloor$ goal vertices 
are filled. Suppose there are $q$ columns in $\mathcal{D}$ with $1\leq f_i\leq m-1$. According 
to the definition of $f_i$, for each of these $q$ columns, there is at least one goal vertex 
that is filled and at least one goal vertex that is not.

If $q< \dfrac{\lfloor n/3 \rfloor}{3(m-1)}$, then there are two columns $i$ and $j$, such that $f_i=m$ and $f_j=0$. That is 
because $\sum_{1\leq i \leq m} f_i= \lfloor n/3 \rfloor$ and $0\leq f_i \leq m$ for all $1\leq i \leq m$. 
Therefore, for the vertex pairs in each row $j$, at least one goal vertex is filled 
but at least one is not. And thus, for each $j$, there are two adjacent columns $i, i+1, 1\leq 
i < m$, such that there is only one goal vertex in $p_{i,j}$ and $p_{i+1,j}$ is filled and the
start vertex in the other vertex pair is cleared (Fig. \ref{fig:LemmaProof}(a)). 
Therefore, there are at least $m$ cleared vertices in this case.

If $q\geq \dfrac{\lfloor n/3 \rfloor}{3(m-1)}$, then we partition all the columns in $\mathcal{D}$ into $\lfloor m/2\rfloor$ disjoint pairs: 
(1,2), (3,4), ... The $q$ columns belong to at least $\lfloor q/2\rfloor$ pairs of 
adjacent columns. Therefore, according to Lemma \ref{lemma:adjacent}, we have $\Theta(m)$ 
cleared vertices.

In conclusion, there are $\Omega(m)$ cleared vertices when there are $\lfloor n/3 \rfloor$ 
filled goal. Therefore, the minimum \mrb of this instance is $\Omega(m)$.
\end{proof}

\begin{proof}[Proof sketch of Theorem~\ref{t:urbm-upper}]
When objects are all uniform cylinders, the corresponding unlabeled dependency graph 
$\udg$ is a planar graph with degree no more than $5$, by 
Proposition~\ref{p:udg}. We propose an $O(n\log(n))$-time algorithm \spp for the 
setting based on a vertex separator of $\udg$. \spp can find a rearrangement plan 
with $ O(\sqrt{n})$ running buffers.

In \spp, given the planar $\udg = (V, E)$, we can partition 
$V$ into three disjoint subsets $A$, $B$ and $C$\cite{lipton1979separator}, such that there is no edge connecting 
vertices in $A$ and $B$, $|A|,|B|\leq 2|V|/3$, and $|C|\leq 2\sqrt{2|V|}$(Fig.~\ref{fig:separator}(a)). For the start vertices in $C$ and the neighbors of the 
goal vertices in $C$, we remove them from $\udg$. Since 
there are at most $5$ neighbors for each goal vertex, there are at most $10\sqrt{2|V|}$ 
objects moved to the buffer in this operation. After that, we remove the goal vertices 
in $C$ which should be isolated now. Let $A'$, $B'$ be the remaining vertices in $A$ 
and $B$. With the removal of $C$ from $\udg$, $A'$ and $B'$ form two independent subgraphs (Fig.~\ref{fig:separator}(b)). We can deal with the subgraphs one after the other by 
recursively calling \spp(Fig.~\ref{fig:separator}(c)). Let $\delta(V'):= g(V')-s(V')$ where 
$g(V')$ and $s(V')$ are the number of goal and start vertices in a vertex set $V'$ 
respectively. Between vertex subsets $A$ and $B$, we prioritize the one with larger $\delta(\cdot)$ value. With 
straightforward reasoning, the $10\sqrt{2|V|}$ upper bound of the additional buffer size 
still holds after we deal with the prioritized subgraph. 
\begin{figure}[h!]
\vspace{2mm}
    \centering
\begin{overpic}
[width=0.45\textwidth]{separator-eps-converted-to.pdf}
\put(12,-5){(a)}
\put(46,-5){(b)}
\put(82,-5){(c)}
\end{overpic}
\vspace{4mm}
    \caption{The recursive solver \spp for \urbm. (a) A $O(\sqrt{|V|})$ vertex separator for the planar dependency graph. (b) By removing the start vertices in $C$ and the neighbors of the goal vertices in $C$, the remaining graph consists of two independent subgraphs and isolated goal poses in $C$. (c) The problem can be solved by recursively calling \spp.}
    \label{fig:separator}
\end{figure}

Let the maximum \rb of the plan found by \spp be $b(m)$, where $m=2n$ is the number of vertices in the 
dependency graph. We have $b(m)\leq b(2m/3)+O(\sqrt{m})$. And therefore, $b(m)=O(\sqrt{m})$. 
Since the $O(\sqrt{|V|})$ vertex separator can be found in $O(|V|)$ time 
\cite{lipton1979separator}, \spp can find the rearrangement plan for an arbitrary $n$-object 
\urbm instance in $O(n\log(n))$ time. Due to limited space, the details of \spp and this proof 
are omitted; they will be made available in the extended version of this paper to be put on arXiv.
\end{proof}

\subsection{Minimizing Total Buffers Subject to \mrb Constraints}\label{subsec:ilp}
Let binary variables $c_{i,j}$ represent $\ldg$: $c_{i,j}=1$ if and only if 
$i=j$ or $(i,j)$ is in the arc set of $\ldg$. Let $y_{i,j}$ be the binary 
sequential variables: $y_{i,j}=1$ if and only if $i=j$ or $o_i$ moves out 
of the start pose before $o_j$. \mrb can be expressed based on three constraints: 
First, \mrb is at least the size of the running buffer at any moment; 
Second, an object $o_j\in \mathcal{O}$ is at the goal pose if and only 
if all the objects $o_k\in \mathcal{O}$ with $c_{j,k}=1$ have left the start 
poses. Third, an object $o_j\in \mathcal{O}$ is at the buffer if and only 
if $o_j$ is neither at the start pose nor at the goal pose.
%
To encode the constraints, we further introduce two sets of binary variables 
$g_{i,j}$ and $b_{i,j}$. $g_{i,j}=1$ and $b_{i,j}=1$ indicate that $o_j$ is at
the goal pose and $o_j$ is at the buffer respectively when the action moving
$o_i$ away from the start pose is complete. Therefore, given a running buffer 
limit $k$, we have:
\vspace{1mm}
\begin{equation}
    k \geq \sum_{1\leq j\leq n} b_{i,j}\ \ \  \forall 1\leq i\leq n
\end{equation}
\begin{equation}
    \sum_{1\leq l \leq n} \dfrac{c_{j,l}y_{i,l}}{n} \leq g_{i,j} \leq \sum_{1\leq l \leq n} c_{j,l}y_{i,l} \ \ \ \forall 1\leq i,j \leq n
\end{equation}
\begin{equation}
\begin{split}
    \sum_{1\leq l \leq n}\dfrac{2-y_{i,l}-g_{i,l}}{2} \leq b_{i,j} \leq \sum_{1\leq l \leq n} (2-y_{i,l}-g_{i,l}) \\ 
    \forall 1\leq i,j \leq n
\end{split}
\end{equation}


%\kg{Perhaps it makes more sense here to use the sum of $b_{i,j}$ to represent the total buffer size rather than adding into Han's formulation.}
\vspace{2mm}
The constraints can be added into the \fvs ILP formulation \cite{han2018complexity} to 
find the minimum total buffer size with at most $k$ running buffers. We denote this method
as $\ilptb$ when $k = \mrb$, and the \fvs method from \cite{han2018complexity} as $\ilpfvs$.

%Therefore, we have 
%two ILP solutions, $\ilpmrb$, which computes solutions optimizing \mrb, and $\ilpfvs$
%which computes the minimum number of total buffers subject to having minimum \mrb.
%Note that even though each vertex $o_i$ are split into $o^{in}_i$ and $o^{out}_i$ in that formulation, the object ordering is indicated by the ordering of $\{o^{in}_i\}_{i=1}^n$.
%\kg{Here I use the ordering of the in-vertices to represent the original object ordering}


